Aspects of the Classical Double Copy

This thesis applies the Kerr-Schild and the Weyl double copy formalisms to study various concepts in the physics literature. First we apply both the Kerr-Schild and the Weyl double copy to solution generating transformations in General Relativity, where we identify Ehlers transformation as the double copy of electromagnetic duality transformation. Secondly, as a spin-off of the Weyl double copy, we use gauge fields defined on curved spacetimes to construct the Weyl tensor and study a host of solution of Einstein's equations. This study provides a test of the non-triviality of the double copy formalism. The second half of the thesis deals with mathematical concepts of physical relevance. First we apply the Kerr-Schild double copy to the concept of holonomy groups of Riemannian manifolds. We find that the single copy of the Riemannian holonomy operator, which we dub SCH, to be a similar operator constructed from the single copy gauge-field curvature. This is followed by a study of this single copy operator on different solutions of Einstein equations and their respective single copies, where we find that the holonomy and SCH groups differ for the Taub-NUT metric, while both reducing to $\text{SU}(2)$ for self-dual solutions. Lastly, we apply the Kerr-Schild double copy to the Ricci flow equation, interpreted as the beta function of the closed string, and obtain the Yang-Mills flow equation, which is physically interpreted as the beta function of the open string coupled to a gauge field.

==> chaps/chap02.tex <==
\chapter{Background material} \label{chap:BG}

